On the convergence of Maronna's $M$-estimators of scatter

In this paper, {we propose an alternative proof for the uniqueness} of Maronna's $M$-estimator of scatter (Maronna, 1976) for $N$ vector observations $\mathbf y_1,...,\mathbf y_N\in\mathbb R^m$ under a mild constraint of linear independence of any subset of $m$ of these vectors. This entails in particular almost sure uniqueness for random vectors $\mathbf y_i$ with a density as long as $N>m$. {This approach allows to establish further relations that demonstrate that a properly normalized Tyler's $M$-estimator of scatter (Tyler, 1987) can be considered as a limit of Maronna's $M$-estimator. More precisely, the contribution is to show that each $M$-estimator converges towards a particular Tyler's $M$-estimator.} These results find important implications in recent works on the large dimensional (random matrix) regime of robust $M$-estimation.

==> definitions.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Distributions, espaces%%%%%%%%%%%%%%%%%
\def\Gr#1{\mathbf #1}
\def\RR{\mathbb{RR}} 
\def\NN{\mathcal{N}}
\def\CN{\mathcal{CN}}
\def\GG{\mathcal{G}}
\def\E{\mathcal{E}}
\def\CE{\mathcal{CE}}
\def\GCE{\mathcal{GCE}}
\def\GCN{\mathcal{GCN}}
\def\WW{\mathcal{W}}
\def\CW{\mathcal{CW}}
\def\S{\mathcal{S}}
%%%%%%%%%%%%%%%%%minuscules en gras%%%%%%%%%%%%%%%%%%%%%
\def\0g{\mathbf{0}}
\def\ag{\mathbf{a}}
\def\bg{\mathbf{b}}
\def\cg{\mathbf{c}}
\def\dg{\mathbf{d}}
\def\eg{\mathbf{e}}
%\def\gg{\mathbf{g}}
\def\kg{\mathbf{k}}
\def\hg{\mathbf{h}}
\def\mg{\mathbf{m}}
\def\ng{\mathbf{n}}
\def\pg{\mathbf{p}}
\def\qg{\mathbf{q}}
\def\sg{\mathbf{s}}
\def\tg{\mathbf{t}}
\def\ug{\mathbf{u}}
\def\vg{\mathbf{v}}
\def\wg{\mathbf{w}}
\def\xg{\mathbf{x}}
\def\yg{\mathbf{y}}
\def\zg{\mathbf{z}}

%%%%%%%%%%%%%%%%%%%lettres grecques en gras%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\alphag{\boldsymbol{\alpha}}
\def\delg{\boldsymbol{\delta}}
\def\mug{\boldsymbol{\mu}}
\def\Dg{\boldsymbol{\Delta}}
\def\Lg{\boldsymbol{\Lambda}}
\def\Pig{\boldsymbol{\Pi}}
\def\Sig{\boldsymbol{\Sigma}}
\def\Gag{\boldsymbol{\Gamma}}
\def\Omg{\boldsymbol{\Omega}}
%%%%%%%%%%%%%%%%%%Majuscules en gras%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Ag{\mathbf{A}}
\def\Bg{\mathbf{B}}
\def\Cg{\mathbf{C}}
\def\Fg{\mathbf{F}}
\def\Gg{\mathbf{G}}
\def\Ig{\mathbf{I}}
\def\Jg{\mathbf{J}}
\def\Kg{\mathbf{K}}
\def\Mg{\mathbf{M}}
\def\Ng{\mathbf{N}}
\def\Pg{\mathbf{P}}
\def\Qg{\mathbf{Q}}
\def\Rg{\mathbf{R}}
\def\Sg{\mathbf{S}}
\def\Tg{\mathbf{T}}
\def\Vg{\mathbf{V}}
\def\Wg{\mathbf{W}}
\def\Wgc{\mathbf{W_c}}
\def\Xg{\mathbf{X}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Lettres avec chapeau%%%%%%%%%%%%%%
\newcommand\Mc{\widehat{\Gr{M}}}
\newcommand\Vc{\widehat{\Gr{V}}}
\newcommand\Rc{\widehat{\Gr{R}}}
\newcommand\Pc{\widehat{\Gr{P}}}
\newcommand\thetac{\widehat{\Gr{\theta}}}
\newcommand\Thetac{\widehat{\Gr{\Theta}}}
\newcommand\Sigc{\widehat{\Gr{\Sigma}}}
\newcommand\bc{\widehat{b}}
\newcommand\varepsilonc{\widehat{\varepsilon}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Lettres avec tilt%%%%%%%%%%%%%%%%%%
\newcommand\At{\overset{\sim}{\Gr{A}}}
\newcommand\Bt{\overset{\sim}{\Gr{B}}}
\newcommand\Mt{\overset{\sim}{\Gr{M}}}
\newcommand\Vt{\overset{\sim}{\Gr{V}}}
\newcommand\Wt{\overset{\sim}{\Gr{W}}}
\newcommand\Wtc{\overset{\sim}{\Gr{W_c}}}
\newcommand\Xt{\overset{\sim}{\Gr{X}}}
\newcommand\att{\overset{\sim}{a}}
\newcommand\bt{\overset{\sim}{b}}
\newcommand\mt{\overset{\sim}{\Gr{m}}}
\newcommand\zt{\overset{\sim}{\Gr{z}}}
\newcommand\wt{\overset{\sim}{w}}
%%%%%%%%%%%%%%%%%%%%%%%%Lettres grecques avec tilt%%%%%%%%%%%%%%%%%%%%
\newcommand\alphagt{\overset{\sim}{\boldsymbol{\alpha}}}
\newcommand\Dt{\overset{\sim}{\boldsymbol{\Lambda}}}
\newcommand\delgt{\overset{\sim}{\boldsymbol{\delta}}}
\newcommand\Sigt{\overset{\sim}{\boldsymbol{\Sigma}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Sections spéciales%%%%%%%%%%%%%%%%%%%%%%
%\newtheorem{Def}{Définition}[section]
%\newtheorem{Thm}{Théorème}[section]
%\newtheorem{Lem}{Lemme}[section]
%\newtheorem{Coro}{Corollaire}[section]
%\newtheorem{Prop}{Proposition}[section]
%\newtheorem{rem}{Remarque}[section]
%\newtheorem{proof}{Preuve}[section]

\newenvironment{Thm}[1]{\vspace{0.5cm}
\fbox{\begin{minipage}{1\linewidth}
\begin{theo}#1\end{theo}\end{minipage}}}{\linebreak}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Parenthèses%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\be{\left(}
\newcommand\bea{\left\{}
\newcommand\bec{\left[}
\newcommand\en{\right)}
\newcommand\ena{\right\}}
\newcommand\enc{\right]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Divers%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\supinf{\underset{H_0}{\overset{H_1}{\gtrless}}}
\newcommand\disp{\displaystyle}
\newcommand\dsum{\displaystyle \sum}
\def\Tr{\,\textup{Tr}}
\def\vec{\textup{vec}}
\def\co{\textup{cov}}
\def\pco{\textup{pcov}}
\def\indic{\mathbbm{1}}
\def\=d{\overset{d}{=}}
\def\>d{\overset{d}{\rightarrow}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Couleurs%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{color}
\definecolor{emeraude}{rgb}{0.5,1,0.75}
\definecolor{vert}{rgb}{0.3,0.7,0.5}
\definecolor{mauve}{rgb}{0.5,0.1,0.9}
\definecolor{rltred}{rgb}{0.75,0,0}
\definecolor{rltgreen}{rgb}{0,0.5,0}
\definecolor{oneblue}{rgb}{0,0,0.75}
\definecolor{marron}{rgb}{0.64,0.16,0.16}
\definecolor{forestgreen}{rgb}{0.13,0.54,0.13}
\definecolor{purple}{rgb}{0.62,0.12,0.94}
\definecolor{dockerblue}{rgb}{0.11,0.56,0.98}
\definecolor{freeblue}{rgb}{0.25,0.41,0.88}
\definecolor{myblue}{rgb}{0,0.2,0.4}
\definecolor{bleuclair}{rgb}{0.6,0.6,0.9}
\definecolor{gris}{rgb}{0.6,0.6,0.6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Macros%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%caption pour minipage contenant figure ou tableaux (avec la bonne numérotation)
\makeatletter
\def\captionof#1#2{{\def\@captype{#1}#2}}
\makeatother
%%%\captionof{figure}{\caption{titre figure}}
%%%\captionof{tableau}{\caption{titre tableau}}
